A unified multimodal understanding and generation model for cross-disciplinary scientific research

Scientific discovery increasingly relies on integrating heterogeneous, high-dimensional data across disciplines nowadays. While AI models have achieved notable success across various scientific domains, they typically remain domain-specific or lack the capability of simultaneously understanding and generating multimodal scientific data, particularly for high-dimensional data. Yet, many pressing global challenges and scientific problems are inherently cross-disciplinary and require coordinated progress across multiple fields. Here, we present FuXi-Uni, a native unified multimodal model for scientific understanding and high-fidelity generation across scientific domains within a single architecture. Specifically, FuXi-Uni aligns cross-disciplinary scientific tokens within natural language tokens and employs science decoder to reconstruct scientific tokens, thereby supporting both natural language conversation and scientific numerical prediction. Empirically, we validate FuXi-Uni in Earth science and Biomedicine. In Earth system modeling, the model supports global weather forecasting, tropical cyclone (TC) forecast editing, and spatial downscaling driven by only language instructions. FuXi-Uni generates 10-day global forecasts at 0.25{\deg} resolution that outperform the SOTA physical forecasting system. It shows superior performance for both TC track and intensity prediction relative to the SOTA physical model, and generates high-resolution regional weather fields that surpass standard interpolation baselines. Regarding biomedicine, FuXi-Uni outperforms leading multimodal large language models on multiple biomedical visual question answering benchmarks. By unifying heterogeneous scientific modalities within a native shared latent space while maintaining strong domain-specific performance, FuXi-Uni provides a step forward more general-purpose, multimodal scientific models.

==> figures/vqa_case/fig_vqa_example_bak.tex <==
% % ---------- helper macro (put here or in preamble) ----------
% \newcommand{\qaimg}[3]{%
%   \begin{minipage}[t]{0.19\textwidth}
%     \centering
%     \includegraphics[height=2.4cm, width=\linewidth, keepaspectratio]{#1}\\[-2pt]
%     {\scriptsize \textbf{Question:}\\
%     \textbf{#2}~#3}
%   \end{minipage}%
% }




% % ---------- figure ----------
% \begin{figure*}[t]
% \centering

% \qaimg{figures/vqa_case/test_1212.jpg}{(1)}{what is present?}\hfill
% \qaimg{figures/vqa_case/test_2913.jpg}{(2)}{what was the abnormal gland from?}\hfill
% \qaimg{figures/vqa_case/test_4279.jpg}{(3)}{Is the dead cell seen in singles?}\hfill
% \qaimg{figures/vqa_case/40464_1.jpg}{(4)}{How would you describe the spleen abnormality?}\hfill
% \qaimg{figures/vqa_case/synpic53033}{(5)}{What side of the brain is a lesion on?}

% \vspace{6pt}

% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.15}

% \begin{tabularx}{\textwidth}{@{}l *{5}{>{\raggedright\arraybackslash}X}@{}}
% \toprule
%  & (1) & (2) & (3) & (4) & (5) \\
% \midrule
% \textbf{Answer} &
% vasculature & a patient with acth-dependent cushing syndrome & yes & right lower lateral lung field & Left \\
% % \textbf{Answer type} &
% % OPEN & OPEN & CLOSED & OPEN & diverticulitis \\
% % \textcolor{blue}{PubMedCLIP} &
% % spinal cord & yes & yes & right lower lateral lung field & diverticulitis \\
% % \textcolor{blue}{BiomedGPT} &
% % coronary artery & female & just one & right lower lateral lung field & diverticulitis \\
% LLaVA\_Tri &
% coronary artery & endocrine system & no & nothing & Right \\
% \textbf{FuXi-Uni} &
% Vasculature & acth-dependent cushing & yes & hypodense lesion & Left \\
% \bottomrule
% \end{tabularx}

% \caption{Examples from VQA-RAD with PubMedCLIP and BiomedGPT.}
% \label{fig:vqa_rad_example}
% \end{figure*}



% ====== basic ======
% \usepackage[margin=1in]{geometry}
% \usepackage{graphicx}

% % ====== table / layout ======
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{array}              % for \arraybackslash
% \usepackage[table]{xcolor}      % for \textcolor
% \usepackage[export]{adjustbox}  % for \adjustbox + valign=t

% ---------- helper macro (put here or in preamble) ----------
% #1: image path
% #2: (1)/(2)/...
% #3: question text

\newcommand{\qaimg}[3]{%
  \begin{minipage}[t]{0.19\textwidth}
    \centering
    % 关键：固定高度 + 顶端对齐；\detokenize 防止路径里有 _ 等特殊字符报错
    \adjustbox{valign=t}{%
      \includegraphics[height=2.4cm,width=\linewidth,keepaspectratio]{\detokenize{#1}}%
    }\\[-2pt]
    {\scriptsize \textbf{Question:}\\
    \textbf{#2}~#3}
  \end{minipage}%
}


% ---------- figure ----------
\begin{figure*}[t]
\centering

\qaimg{figures/vqa_case/test_1212.jpg}{(1)}{what is present?}\hfill
\qaimg{figures/vqa_case/test_2913.jpg}{(2)}{what was the abnormal gland from?}\hfill
\qaimg{figures/vqa_case/test_4279.jpg}{(3)}{Is the dead cell seen in singles?}\hfill
\qaimg{figures/vqa_case/40464_1.jpg}{(4)}{How would you describe the spleen abnormality?}\hfill
\qaimg{figures/vqa_case/synpic53033.jpg}{(5)}{What side of the brain is a lesion on?}

\vspace{6pt}

\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabularx}{\textwidth}{@{}l *{5}{>{\raggedright\arraybackslash}X}@{}}
\toprule
 & (1) & (2) & (3) & (4) & (5) \\
\midrule
\textbf{Answer} &
vasculature & a patient with acth-dependent cushing syndrome & yes & right lower lateral lung field & Left \\
\textcolor{blue}{LLaVA\_Tri} &
coronary artery & endocrine system & no & nothing & Right \\
\textcolor{red}{FuXi-Uni} &
Vasculature & acth-dependent cushing & yes & hypodense lesion & Left \\
\bottomrule
\end{tabularx}

\caption{Examples from VQA-RAD with PubMedCLIP and BiomedGPT.}
\label{fig:vqa_rad_example}
\end{figure*}


==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
